The ASAS-SN Bright Supernova Catalog -- V. 2018-2020

We catalog the 443 bright supernovae discovered by the All-Sky Automated Survey for Supernovae (ASAS-SN) in $2018-2020$ along with the 519 supernovae recovered by ASAS-SN and 516 additional $m_{peak}\leq18$ mag supernovae missed by ASAS-SN. Our statistical analysis focuses primarily on the 984 supernovae discovered or recovered in ASAS-SN $g$-band observations. The complete sample of 2427 ASAS-SN supernovae includes earlier $V$-band samples and unrecovered supernovae. For each supernova, we identify the host galaxy, its UV to mid-IR photometry, and the offset of the supernova from the center of the host. Updated light curves, redshifts, classifications, and host galaxy identifications supersede earlier results. With the increase of the limiting magnitude to $g\leq18$ mag, the ASAS-SN sample is roughly complete up to $m_{peak}=16.7$ mag and is $90\%$ complete for $m_{peak}\leq17.0$ mag. This is an increase from the $V$-band sample where it was roughly complete up to $m_{peak}=16.2$ mag and $70\%$ complete for $m_{peak}\leq17.0$ mag.

==> authors.tex <==
%% Plain Authors (outdated backup)
\author[K.~D.~Neumann et al.]{K.~D.~Neumann$^{1}$\thanks{neumann.110@osu.edu}, T.~W.-S.~Holoien$^{2}$, C.~S.~Kochanek$^{1,3}$, K.~Z.~Stanek$^{1,3}$,
\newauthor
P.~J.~Vallely$^{1}$, 
B.~J.~Shappee$^{4}$, 
J.~L.~Prieto$^{5,6}$, 
T.~Pessi$^{5,7}$, 
T.~Jayasinghe$^{8,1,\dagger}$, 
\newauthor
J.~Brimacombe$^{9}$, 
D.~Bersier$^{10}$, 
E.~Aydi$^{11,\dagger}$, 
C.~Basinger$^{1}$, 
J.~F.~Beacom$^{3,12,1}$, 
\newauthor
S.~Bose$^{13}$, 
J.~S.~Brown$^{1,14}$, 
P.~Chen$^{15}$, 
A.~Clocchiatti$^{16}$, 
D.~D.~Desai$^{4}$, 
S.~Dong$^{13}$, 
\newauthor
E.~Falco$^{17}$, 
S.~Holmbo$^{18}$, 
N.~Morrell$^{19}$, 
J.~V.~Shields$^{20}$, 
K.~Sokolovsky$^{11,21}$, 
\newauthor
J.~Strader$^{11}$, 
M.~D.~Stritzinger$^{18}$, 
S.~Swihart$^{22}$, 
T.~A.~Thompson$^{1,3}$, 
Z.~Way$^{23}$, 
\newauthor
L.~Aslan$^{2}$, 
D.~W.~Bishop$^{24}$, 
G.~Bock$^{25}$, 
J.~Bradshaw$^{26}$, 
P.~Cacella$^{27}$, 
N.~Castro$^{6}$,
\newauthor
E.~Conseil$^{28}$, 
R.~Cornect$^{29}$, 
I.~Cruz$^{30}$, 
R.~G.~Farfan$^{31,32}$, 
J.~M.~Fernandez$^{33,32}$, 
\newauthor
A.~Gabuya$^{34}$, 
J.-L.~Gonzalez-Carballo$^{35,32,36}$, 
M.~ R.~Kendurkar$^{37}$, 
S.~Kiyota$^{38}$, 
\newauthor
R.~A.~Koff$^{39}$, 
G.~Krannich$^{40}$, 
P.~Marples$^{41}$, 
G.~Masi$^{42}$, 
L.~A.~G.~Monard$^{43}$, 
\newauthor
J.~A.~Mu\~{n}oz$^{44,45}$, 
B.~Nicholls$^{46}$, 
R.~S.~Post$^{47}$, 
Z.~Pujic$^{48}$, 
G.~Stone$^{49}$, 
L.~Tomasella$^{50}$, 
\newauthor
D.~L.~Trappett$^{51}$, 
W.~S.~Wiethoff$^{52}$ \\
\vspace{0.4cm}
\\
\parbox{\textwidth}{
(affiliations are listed at the end of the paper)\\
}
}
%%%%%% Should I move these to the end of the paper? Before/After Acknowledgments
  $^{1}$ Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA \\
  $^{2}$ The Observatories of the Carnegie Institution for Science, 813 Santa Barbara Street, Pasadena, CA 91101, USA \\
  $^{3}$ Center for Cosmology and AstroParticle Physics (CCAPP), The Ohio State University, 191 W. Woodruff Ave., Columbus, OH 43210, USA \\
  $^{4}$ Institute for Astronomy, University of Hawai'i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA \\
  $^{5}$ N\'ucleo de Astronom\'ia de la Facultad de Ingenier\'ia y Ciencias, Universidad Diego Portales, Av. Ej\'ercito 441, Santiago, Chile \\
  $^{6}$ MAS, Millennium Institute of Astrophysics, Santiago, Chile \\
  $^{7}$ European Southern Observatory, Alonso de C\'ordova 3107, Casilla 19, Santiago, Chile \\
  $^{8}$ Department of Astronomy, University of California Berkeley, Berkeley CA 94720, USA \\
  $^{9}$ Coral Towers Observatory, Cairns, Queensland 4870, Australia \\
  $^{10}$ Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK \\
  $^{11}$ Center for Data Intensive and Time Domain Astronomy, Department of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA \\
  $^{12}$ Department of Physics, The Ohio State University, 191 W. Woodruff Ave., Columbus, OH 43210, USA \\
  $^{13}$ Kavli Institute for Astronomy and Astrophysics, Peking University, Yi He Yuan Road 5, Hai Dian District, Beijing 100871, China \\
  $^{14}$ Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 92064, USA \\
  $^{15}$ Department of Particle Physics and Astrophysics, Weizmann Institute of Science, 234 Herzl St, 7610001 Rehovot, Israel \\
  $^{16}$ Instituto de Astrofísica, Pontificia Universidad Catolica de Chile, Instituto Milenio de Astrofisica (MAS), Vicuna Mackenna 4860, Macul, Santiago, Chile\\
  $^{17}$ Harvard-Smithsonian Center for Astrophysics, 60 Garden St., Cambridge, MA 02138, USA \\
  $^{18}$ Department of Physics and Astronomy, Aarhus University, Ny Munkegade 120, DK-8000 Aarhus C, Denmark \\
  $^{19}$ Las Campanas Observatory, Carnegie Observatories, Casilla 601, La Serena, Chile \\
  $^{20}$ Department of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA \\
  $^{21}$ Sternberg Astronomical Institute, Moscow State University, Universitetskii pr. 13, 119992 Moscow, Russia \\
  $^{22}$ National Research Council Research Associate, National Academy of Sciences, Washington, DC 20001, USA, resident at Naval Research Laboratory, Washington, DC 20375, USA \\
  $^{23}$ Physics & Astronomy Department, Georgia State University, 25 Park Place, Atlanta, GA 30302, USA \\
  $^{24}$ Rochester Academy of Science, 1194 West Avenue, Hilton, NY 14468, USA \\
  $^{25}$ Runaway Bay Observatory, 1 Lee Road, Runaway Bay, Queensland 4216, Australia \\
  $^{26}$ Samford Valley Observatory (Q79), Queensland, 4520, Australia \\
  $^{27}$ DogsHeaven Observatory, SMPW Q25 CJ1 LT10, Brasilia, DF 71745-501, Brazil \\
  $^{28}$ Association Francaise des Observateurs d'Etoiles Variables (AFOEV), Observatoire de Strasbourg, 11 Rue de l'Universite, France \\
  $^{29}$ Moondyne Observatory, 61 Moondyne Rd, Mokine, WA 6401, Australia \\
  $^{30}$ Slate Ridge Observatory, 1971 Haverton Drive, Reynoldsburg, OH 43068, USA \\
  $^{31}$ Observatorio Uraniborg, MPC Z55, Ecija, Sevilla, Spain \\
  $^{32}$ Observadores de Supernovas (ObSN), Spain \\
  $^{33}$ Observatory Inmaculada del Molino, Sevilla, Spain \\
  $^{34}$ Al Sadeem Observatory, Al Wathba South, Abu Dhabi, UAE \\
  $^{35}$ Observatorio Cerro del Viento-MPC I84, Badajoz, Spain \\
  $^{36}$ AAVSO, 185 Alewife Brook Parkway, Suite 410, Cambridge, MA 02138, USA \\
  $^{37}$ Prince George Astronomical Observatory, 7365 Tedford, Prince George, BC V2N 6S2, Canada \\
  $^{38}$ Variable Star Observers League in Japan, 7-1 Kitahatsutomi, Kamagaya, Chiba 273-0126, Japan \\
  $^{39}$ Antelope Hills Observatory, 980 Antelope Drive West, Bennett, CO 80102, USA \\
  $^{40}$ Roof Observatory Kaufering, Lessingstr. 16, D-86916 Kaufering, Germany \\
  $^{41}$ Peter Observatory, unit 316 Sandcastles 392 Marine Pde, Labrador, Qld 4215, Australia \\
  $^{42}$ Virtual Telescope Project, Via Madonna de Loco, 47-03023 Ceccano (FR), Italy \\
  $^{43}$ Kleinkaroo Observatory, Calitzdorp, St. Helena 1B, P.O. Box 281, 6660 Calitzdorp, Western Cape, South Africa \\
  $^{44}$ Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universidad de Valencia, E-46100 Burjassot, Valencia, Spain \\
  $^{45}$ Observatorio Astron\'omico, Universidad de Valencia, E-46980 Paterna, Valencia, Spain \\
  $^{46}$ Mount Vernon Observatory, 6 Mount Vernon Place, Nelson, New Zealand \\
  $^{47}$ Post Observatory, Lexington, MA 02421, USA \\
  $^{48}$ Alexander Observatory, Brisbane, Australia \\
  $^{49}$ First Light Observatory Systems, 17908 NE 391st St, Amboy, WA 98601, USA \\
  $^{50}$ INAF – Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122 Padova, Italy \\
  $^{51}$ Brisbane Girls Grammar School - Dorothy Hill Observatory, Gregory Terrace, Spring Hill, Queensland 4000, Australia \\
  $^{52}$ Department of Earth and Environmental Sciences, University of Minnesota, 230 Heller Hall, 1114 Kirby Drive, Duluth, MN. 55812, USA \\
 

==> authors_orcid.tex <==
%% Authors with ORCID (backup)
\author[K.~D.~Neumann et al.]{K.~D.~Neumann \orcidlink{0000-0002-2701-8433}$^{1}$\thanks{neumann.110@osu.edu}, 
T.~W.-S.~Holoien \orcidlink{0000-0001-9206-3460}$^{2}$, 
C.~S.~Kochanek$^{1,3}$, 
K.~Z.~Stanek$^{1,3}$, 
\newauthor
P.~J.~Vallely$^{1}$, 
B.~J.~Shappee \orcidlink{0000-0003-4631-1149}$^{4}$, 
J.~L.~Prieto$^{5,6}$, 
T.~Pessi \orcidlink{0000-0001-6540-0767}$^{5,7}$, 
T.~Jayasinghe \orcidlink{0000-0002-6244-477X}$^{8,1,\dagger}$, 
\newauthor
J.~Brimacombe$^{9}$, 
D.~Bersier \orcidlink{0000-0001-7485-3020}$^{10}$, 
E.~Aydi \orcidlink{0000-0001-8525-3442}$^{11,\dagger}$, 
C.~Basinger$^{1}$, 
J.~F.~Beacom \orcidlink{0000-0002-0005-2631}$^{3,12,1}$, 
\newauthor
S.~Bose \orcidlink{0000-0003-3529-3854}$^{13}$, 
J.~S.~Brown$^{1,14}$, 
P.~Chen \orcidlink{0000-0003-0853-6427}$^{15}$, 
A.~Clocchiatti \orcidlink{0000-0003-3068-4258}$^{16}$, 
D.~D.~Desai \orcidlink{0000-0002-2164-859X}$^{4}$, 
\newauthor
Subo~Dong \orcidlink{0000-0002-1027-0990}$^{13}$, 
E.~Falco \orcidlink{0000-0002-7061-6519}$^{17}$, 
S.~Holmbo \orcidlink{0000-0002-3415-322X}$^{18}$, 
N.~Morrell \orcidlink{0000-0003-2535-3091}$^{19}$, 
J.~V.~Shields \orcidlink{0000-0002-1560-5286}$^{20}$, 
\newauthor
K.~V.~Sokolovsky \orcidlink{0000-0001-5991-6863}$^{11,21}$, 
J.~Strader \orcidlink{0000-0002-1468-9668}$^{11}$, 
M.~D.~Stritzinger \orcidlink{0000-0002-5571-1833}$^{18}$, 
S.~Swihart \orcidlink{0000-0003-1699-8867}$^{22}$, 
\newauthor
T.~A.~Thompson \orcidlink{0000-0003-2377-9574}$^{1,3}$, 
Z.~Way \orcidlink{0000-0003-0179-9662}$^{23}$, 
L.~Aslan$^{2}$, 
D.~W.~Bishop$^{24}$, 
G.~Bock$^{25}$, 
\newauthor
J.~Bradshaw$^{26}$, 
P.~Cacella \orcidlink{0000-0002-3546-3190}$^{27}$, 
N.~Castro-Morales$^{16}$, 
E.~Conseil$^{28}$, 
R.~Cornect$^{29}$, 
\newauthor
I.~Cruz$^{30}$, 
R.~G.~Farfan$^{31,32}$, 
J.~M.~Fernandez$^{33,32}$, 
A.~Gabuya \orcidlink{0000-0003-1541-7557}$^{34}$, 
\newauthor
J.-L.~Gonzalez-Carballo$^{35,32,36}$, 
M.~ R.~Kendurkar$^{37}$, 
S.~Kiyota \orcidlink{0000-0003-2694-7692}$^{38}$, 
R.~A.~Koff$^{39}$,
\newauthor
G.~Krannich$^{40}$, 
P.~Marples$^{41}$, 
G.~Masi$^{42}$, 
L.~A.~G.~Monard$^{43}$, 
J.~A.~Mu\~{n}oz \orcidlink{0000-0001-9833-2959}$^{44,45}$, 
\newauthor
B.~Nicholls$^{46}$, 
R.~S.~Post \orcidlink{0000-0003-3244-0337}$^{47}$, 
Z.~Pujic \orcidlink{0000-0002-2515-7296}$^{48}$, 
G.~Stone \orcidlink{0000-0001-5888-9162}$^{49}$, 
L.~Tomasella \orcidlink{0000-0002-3697-2616}$^{50}$, 
\newauthor
D.~L.~Trappett$^{51}$, 
W.~S.~Wiethoff$^{52}$ \\
\vspace{0.4cm}
\\
\parbox{\textwidth}{
Affiliations are listed at the end of the paper\\
$^{\dagger}$ NASA Hubble Fellow \\
    }
 } 
  $^{0}$ NASA Hubble Fellow \\
    $^{1}$ Department of Astronomy, The Ohio State University, 140 West 18th Avenue, Columbus, OH 43210, USA \\
  $^{2}$ The Observatories of the Carnegie Institution for Science, 813 Santa Barbara Street, Pasadena, CA 91101, USA \\
  $^{3}$ Center for Cosmology and AstroParticle Physics (CCAPP), The Ohio State University, 191 W. Woodruff Ave., Columbus, OH 43210, USA \\
  $^{4}$ Institute for Astronomy, University of Hawai'i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA \\
  $^{5}$ N\'ucleo de Astronom\'ia de la Facultad de Ingenier\'ia y Ciencias, Universidad Diego Portales, Av. Ej\'ercito 441, Santiago, Chile \\
  $^{6}$ MAS, Millennium Institute of Astrophysics, Santiago, Chile \\
  $^{7}$ European Southern Observatory, Alonso de C\'ordova 3107, Casilla 19, Santiago, Chile \\
  $^{8}$ Department of Astronomy, University of California Berkeley, Berkeley CA 94720, USA \\
  $^{9}$ Coral Towers Observatory, Cairns, Queensland 4870, Australia \\
  $^{10}$ Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK \\
  $^{11}$ Center for Data Intensive and Time Domain Astronomy, Department of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA \\
  $^{12}$ Department of Physics, The Ohio State University, 191 W. Woodruff Ave., Columbus, OH 43210, USA \\
  $^{13}$ Kavli Institute for Astronomy and Astrophysics, Peking University, Yi He Yuan Road 5, Hai Dian District, Beijing 100871, China \\
  $^{14}$ Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 92064, USA \\
  $^{15}$ Department of Particle Physics and Astrophysics, Weizmann Institute of Science, 234 Herzl St, 7610001 Rehovot, Israel \\
  $^{16}$ Instituto de Astrofísica, Pontificia Universidad Catolica de Chile, Instituto Milenio de Astrofisica (MAS), Vicuna Mackenna 4860, Macul, Santiago, Chile\\
  $^{17}$ Harvard-Smithsonian Center for Astrophysics, 60 Garden St., Cambridge, MA 02138, USA \\
  $^{18}$ Department of Physics and Astronomy, Aarhus University, Ny Munkegade 120, DK-8000 Aarhus C, Denmark \\
  $^{19}$ Las Campanas Observatory, Carnegie Observatories, Casilla 601, La Serena, Chile \\
  $^{20}$ Department of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA \\
  $^{21}$ Sternberg Astronomical Institute, Moscow State University, Universitetskii pr. 13, 119992 Moscow, Russia \\
  $^{22}$ National Research Council Research Associate, National Academy of Sciences, Washington, DC 20001, USA, resident at Naval Research Laboratory, Washington, DC 20375, USA \\
  $^{23}$ Physics & Astronomy Department, Georgia State University, 25 Park Place, Atlanta, GA 30302, USA \\
  $^{24}$ Rochester Academy of Science, 1194 West Avenue, Hilton, NY 14468, USA \\
  $^{25}$ Runaway Bay Observatory, 1 Lee Road, Runaway Bay, Queensland 4216, Australia \\
  $^{26}$ Samford Valley Observatory (Q79), Queensland, 4520, Australia \\
  $^{27}$ DogsHeaven Observatory, SMPW Q25 CJ1 LT10, Brasilia, DF 71745-501, Brazil \\
  $^{28}$ Association Francaise des Observateurs d'Etoiles Variables (AFOEV), Observatoire de Strasbourg, 11 Rue de l'Universite, France \\
  $^{29}$ Moondyne Observatory, 61 Moondyne Rd, Mokine, WA 6401, Australia \\
  $^{30}$ Slate Ridge Observatory, 1971 Haverton Drive, Reynoldsburg, OH 43068, USA \\
  $^{31}$ Observatorio Uraniborg, MPC Z55, Ecija, Sevilla, Spain \\
  $^{32}$ Observadores de Supernovas (ObSN), Spain \\
  $^{33}$ Observatory Inmaculada del Molino, Sevilla, Spain \\
  $^{34}$ Al Sadeem Observatory, Al Wathba South, Abu Dhabi, UAE \\
  $^{35}$ Observatorio Cerro del Viento-MPC I84, Badajoz, Spain \\
  $^{36}$ AAVSO, 185 Alewife Brook Parkway, Suite 410, Cambridge, MA 02138, USA \\
  $^{37}$ Prince George Astronomical Observatory, 7365 Tedford, Prince George, BC V2N 6S2, Canada \\
  $^{38}$ Variable Star Observers League in Japan, 7-1 Kitahatsutomi, Kamagaya, Chiba 273-0126, Japan \\
  $^{39}$ Antelope Hills Observatory, 980 Antelope Drive West, Bennett, CO 80102, USA \\
  $^{40}$ Roof Observatory Kaufering, Lessingstr. 16, D-86916 Kaufering, Germany \\
  $^{41}$ Peter Observatory, unit 316 Sandcastles 392 Marine Pde, Labrador, Qld 4215, Australia \\
  $^{42}$ Virtual Telescope Project, Via Madonna de Loco, 47-03023 Ceccano (FR), Italy \\
  $^{43}$ Kleinkaroo Observatory, Calitzdorp, St. Helena 1B, P.O. Box 281, 6660 Calitzdorp, Western Cape, South Africa \\
  $^{44}$ Departamento de Astronom\'{\i}a y Astrof\'{\i}sica, Universidad de Valencia, E-46100 Burjassot, Valencia, Spain \\
  $^{45}$ Observatorio Astron\'omico, Universidad de Valencia, E-46980 Paterna, Valencia, Spain \\
  $^{46}$ Mount Vernon Observatory, 6 Mount Vernon Place, Nelson, New Zealand \\
  $^{47}$ Post Observatory, Lexington, MA 02421, USA \\
  $^{48}$ Alexander Observatory, Brisbane, Australia \\
  $^{49}$ First Light Observatory Systems, 17908 NE 391st St, Amboy, WA 98601, USA \\
  $^{50}$ INAF – Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122 Padova, Italy \\
  $^{51}$ Brisbane Girls Grammar School - Dorothy Hill Observatory, Gregory Terrace, Spring Hill, Queensland 4000, Australia \\
  $^{52}$ Department of Earth and Environmental Sciences, University of Minnesota, 230 Heller Hall, 1114 Kirby Drive, Duluth, MN. 55812, USA \\
  
